Deep Search Query Intent Understanding

Understanding a user's query intent behind a search is critical for modern search engine success. Accurate query intent prediction allows the search engine to better serve the user's need by rendering results from more relevant categories. This paper aims to provide a comprehensive learning framework for modeling query intent under different stages of a search. We focus on the design for 1) predicting users' intents as they type in queries on-the-fly in typeahead search using character-level models; and 2) accurate word-level intent prediction models for complete queries. Various deep learning components for query text understanding are experimented. Offline evaluation and online A/B test experiments show that the proposed methods are effective in understanding query intent and efficient to scale for online search systems.

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

==> graveyard.tex <==



\begin{comment}
Understanding the query intent in web search involves identifying or categorizing the users’ informational need, in other words, what the users want to find with the searched queries. %
Traditionally, researchers focus on three types of general intents:  informational, navigational, transactional \cite{broder2002taxonomy,jansen2007determining}. Recently, more fine-grained intents are defined \cite{}. For example, for a LinkedIn query that contains keywords \texttt{machine learning}, users could be looking for machine learning jobs, connections with machine learning skills, or online courses to learn machine learning, etc.


Understanding the intent of a searcher is crucial to the success of search systems. Query, contains rich textual information provided by the searcher, is a strong indicator to the searcher’s intent. Understanding the underlying searcher intent from a query, is a referred to the task of query intent modeling.


Query intent is an important component in the search engine ecosystem \cite{kang2003query,li2008learning,hu2009understanding}. As shown in Figure \ref{}, intent is predicted based on incomplete queries when user starts typing; when user finishes typing the whole query, a more accurate intent is predicted based on the completed query.  Accurately understanding user's informational need accurately allows the search engine to trigger corresponding vertical searches, as well as rank the retrieved documents based on the intent \cite{arguello2009sources}, so that users do not have to refine their queries by navigating through the different facets in the search engine. 
%For example, in Figure \ref{}, query intent is identified for the typeahead blending, when the query is incomplete; when user hit 

%Query intent is also beneficial i \cite{ashkan2009classifying}, where advertisements could be  highly relevant to the user intent, which makes the advertisements less intrusive. 


% Challenges

% This could be a challenging task in two aspects. First of all, 
% intent could be ambiguous and subjective. This poses difficulties in labeled data collection. Collecting human-labeled data is time and resource consuming and requires strictly defined rules for quality control. Since intent could be subjective to different users, it would be difficult for raters to label the vertical intents based on search queries. 
% Another challenge this brings is that the vertical intent could be different for the same queries. For search queries like "LinkedIn Jobs," the intent is clear that the user is most likely looking for \textit{job} results. However, a large portion of the search traffic is composed of queries whose intent is not as clear. An example is "software engineer": it could be that the user is a recruiter looking for possible candidates for certain jobs, or could be a job seeker searching for job opportunities. 

Several challenges exist in query intent identification. First of all, unlike sentences in other classic NLP tasks \cite{}, queries are has much \textbf{smaller context}, usually two or three words in a query. Bag-of-Words based approaches fail at capturing the underlying semantics. For example, \texttt{Steve Jobs} refers to a person intent, not a type of job posts; \texttt{san francisco openings} has a job type intent, while \texttt{restaurant opening} refers to a skill. To this end, deep learning methods can identify similar word meanings, and perform sense disambiguation by generating contextualized word embedding.

The short context poses another challenge: given the query words, the intent is usually \textbf{ambiguous}. An example is \texttt{software engineer in machine learning}; it could be that the member is a recruiter looking for possible candidates for machine learning positions, or it could be a job seeker searching for machine learning job opportunities.  Therefore, in this work, we show how to extract effective user behavior features and integrate them into the deep learning framework of query intent.

Motivated by the two challenges, we design a practical deep learning framework for query intent understanding, which is integrated into LinkedIn's commercial search engines. We identified two search result blending components where query intent could be useful: typeahead blending and SERP blending (search engine result page). As shown in Figure \ref{}, the query intent is detected when users are typing each character.  Based on the incomplete queries, the 


% Besides the ambiguity nature of search query intent, different search product calls for different model input and architecture. In text classification, both word representation and character representation have been proven to be effective under different scenarios. Deep learning based word representation models have achieved significant improvements. CNN, as an example, is powerful at capturing the spatial relationships given the word representation of the query text to be classified. Word representations generally preserves important semantics better than character level representations. However, it also has noticeable limitations as the vocabulary of such models are fixed, therefore lacking flexibility of handling out-of-vocabulary (OOV) words. Character level representations, on the other hand, uses characters as vocabulary words, which results in a small yet general vocabulary. Character embedding is effective at handling OOV words as it learns the orthographic information in text. Character level classification models usually use less parameters, and are good at handling short texts as input.
 
 
This paper is motivated by tackling the challenges in query intent prediction tasks, while satisfying production needs in order to achieve real-world impact in search systems. The major contributions are:
\begin{itemize}
    \item A comprehensive introduction of query intent models in a real-world search engine. We share why query intent is important in search, and how the results of query intent are leveraged in search result blending. 
    \item For intent modeling in typeahead, before the queries are complete, we design per-language as well as multilingual character-level models. To our best knowledge, this is the first character-level query intent model. 
    \item We also design several word-level intent prediction models for completed queries which are leveraged in search result page blending. We have experimented with CNN-based and BERT-based models. To our best knowledge, this is the first attempt to incorporate BERT for search query intent prediction problems. 
\end{itemize}

In the rest of this paper, we first introduce how query intent is defined and utilized in LinkedIn search products. This is followed by the design of different granularity (character/word-level) models to adapt to different stages of intent prediction.  The experiments and results show that the proposed deep learning based character/word-level representation models are effective at understanding users' search intents as well as efficient for productionalization in online search systems.

\end{comment}



\begin{comment}
\section{Query Intent Understanding at LinkedIn}

% What is query intent at LinkedIn?
% Why we need query intent at LinkedIn?  Where is it applied (search blending, typeahead blending)?



LinkedIn powers multiple products under the world's largest professional network. Different types of entities exist for different products: user's profile pages for \textit{people} search, job description page for \textit{job} search, news articles and feeds for \textit{content} search, etc. Understanding the intent behind a search is crucial for LinkedIn search success as a correct intent prediction leads to more relevant results for the search result page rendered to the user. 

At LinkedIn, there are two types of searches: vertical search and top page search.

\begin{figure}
\begin{subfigure}{0.23\textwidth}
\includegraphics[width=\linewidth]{figure/people.PNG}
\caption{\textit{People} Search} \label{figure:people-search}
\end{subfigure}
\begin{subfigure}{0.23\textwidth}
\includegraphics[width=\linewidth]{figure/job.PNG}
\caption{\textit{Job} Search} \label{figure:job-search}
\end{subfigure}
\hspace*{\fill} % separation between the subfigures
\caption{Vertical search examples.} 
\label{figure:vertical_search}
\end{figure}

A vertical search is when a user explicitly specify the vertical he/she refers to when the query is searched. For example, the top two verticals that receives the most traffic is \textit{people} search and \textit{job} search. In \textit{people} search, all results retrieved are people entities (user profile pages), whereas in \textit{job} search the results are job description pages.  

Top page search, or top search, refers to a search issued from the global header at LinkedIn.com, without any vertical information specified. Unlike vertical searches, a fundamental challenge is that the search engine lacks the explicit information about users' intents towards the different types of entities in top search. It also needs to render a blended search result page to the user with the relevant results ranked according to the intent behind the search. Therefore, query intent understanding is strongly needed for delivering relevant search results at LinkedIn top page search.

Top page searches could be further categorized into two types: traditional search and typeahead search. Traditional search refers to when a search query is completely typed and the user submits the search. Typeahead search, different from traditional search, provides search results as the user type in. The results in the drop down menu below the search bar could change with every key press. Query intent understanding is applied to both traditional search and typeahead search. 

\begin{figure*}
  \includegraphics[width=120mm]{figure/qim-flow.pdf}
  \caption{Dynamic query intent prediction in search.}
  \label{figure:qim-flow}
\end{figure*}

\subsection{Query Intent in LinkedIn Search System}
% Query reformulation and tokenization
% Query understanding <- intent
% Vertical selection
% Search result blending

We introduce the high-level ecosystem of LinkedIn search, focusing on how query intent prediction is used throughout. When a user types in a query in the search bar, the query is first processed through query reformulation and tokenization. These steps (e.g. spell check, query suggestion, autocomplete suggestion, language detection) provide the fundamental query preprocessing for downstream tasks. 
The next step is further understanding the query and providing language features based on the query string and context. Query intent prediction is one of the components in query understanding. The outcome of query intent understanding is a set of probabilities over different intents. This is an important indicator for what kinds of information the user wants to find with the searched query and is leveraged in succeeding modules. 
In the next stage, the results ranked from vertical searches are returned and blended together in the aggregated search result page and rendered to the users. A key feature for this component is the query intent predictions, which models the direct intents explicitly expressed with the query. Besides the query features, other features are also used to facilitate the accurate selection of search verticals. These include: 1) retrieved document relevance features, 2) query-document matching features, 3) member characteristics and history behavioral features.  This high-level view of the search system at LinkedIn shows how query intent understanding is used to provide a blended page of quality search results to the users.

In the following subsections, we'll introduce the details of how query intent are integrated during different stages of a search.

\begin{figure}
\begin{subfigure}{0.23\textwidth}
\includegraphics[width=\linewidth]{figure/tra_top.PNG}
\caption{Traditional Search} \label{figure:tra_top}
\end{subfigure}
\begin{subfigure}{0.23\textwidth}
\includegraphics[width=\linewidth]{figure/tyah_top.PNG}
\caption{Typeahead Search} \label{figure:tyah_top}
\end{subfigure}
\hspace*{\fill} % separation between the subfigures
\caption{Top page search examples.} \label{figure:top_search}
\end{figure}


\subsection{Query Intent in Typeahead}
 Typeahead search has been widely used in modern search engines. Many advanced typeahead search engines give not only the query auto-complete suggestion, but also the relevant entity results in the drop down menu as shortcuts to relevant/promoted items. 
 As soon as the user start typing in the search box, intent is formed even though the complete information is not yet available. Initial understanding of the intent with queries in the incomplete stage could still benefit typeahead search rendering as the entire process of understanding the intents becomes more accurate as the user continue to type.  The major difference between typeahead search and traditional search is that in typeahead search, results are incrementally changing with each key press. This means that the queries that the search engine use for retrieval is incomplete most of the times. 

The typeahead search results are blended in a similar fashion as in the traditional search. Query intent understanding is also crucial in determining the rank of the different categories of results. For example, query \texttt{lin} might suggest result page of a connection named \texttt{linda} as this keyword is a common subword of names. As the user keeps typing and reached the query \texttt{linked}, the company pages related to \texttt{LinkedIn} should be of great confidence. 

Query intent for typeahead blending is very challenging given that the queries are often incomplete and bears less information than complete words. Therefore it requires a significantly large vocabulary compared to traditional search blending. In addition, the typeahead result rendering is near real time and requires a much smaller latency compared to traditional search. This calls for a lightweight model with good relevance performance.

\subsection{Intent Understanding with Completed Queries}
% What's traditional search
% How's the results blended
% Why is qim needed
% Challenges

As mentioned previously, a traditional search refers to when a user types in a complete query and submits the search. The result page of the search is a set of blended results ranked by a machine learnt ranking model. The quality of the search result blending directly affects user experience on LinkedIn. 

% Why are results blended on SERP?
Since the search engine do not receive any explicit information about within which vertical/product the user is interested in searching, a blending strategy is strongly called for to provide better user experience when searching on LinkedIn. Search queries are usually short and contain wide range of ambiguity. Providing a Search Engine Result Page (SERP) with results from different verticals instead of a single vertical gives a wider range of relevant results. For example, for the query \texttt{google}, the user could be looking for the company Google, or people from Google, or job opportunities from Google. 

How are the search results blended? 
There two types of entities/results in LinkedIn SERP: primary result and secondary results. Each returned SERP has only one primary result type, which is the type of result that the user most likely is searching for. The secondary results contains entities/results from other relevant verticals, which should also be shown to the users for better recall and ambiguity alleviation. Secondary results from the same vertical/product are grouped together and these groups are rendered as carousals in between the primary results to the users. Providing an accurate understanding of the vertical/product intents of a query is crucial for a success search blending. 

Several challenges exist in traditional search blending. 1) Search queries are short yet contain complex semantics. 2) Query intent is very subjective. A job seeker searching with the query \texttt{LinkedIn} is more likely searching with \textit{job} intent, while a recruiter with the same query might suggests a \textit{people} search. 3) Ambiguity is a significant problem. \texttt{LinkedIn Jobs} and \texttt{Steve Jobs} both contains the word \texttt{jobs}, yet bear very different meanings. This calls for understanding the contextual information within the queries.
\end{comment}






% \section{Word-level Model for Search Blending}
% In this section, we describe our approach of learning a word-level query intent prediction model. 

% \subsection{Intent and Label Data Collection}
% \label{section:label-data}
% One of the challenges in query intent modeling is the lack of ground-truth data. First of all, a clear definition of search query intent is difficult to achieve. For queries like "stanford university", we could interpret this is the case where a user wants to find the school Stanford University. However, the user may also want to look for people who graduated from the university or who're working at Stanford. Therefore designing rules for labeling the queries with different intent classes is a challenging task. 
% Secondly, intent is subjective, meaning that the intent for queries could vary in users of different background or even the same users but under different circumstances.For example, a job seeker searching with query "linkedin machine learning" could have strong intent looking for job posting results, whereas a recruiter searching with the same query hopes to get more profile pages as results. This means when labeling search queries with vertical intents, it's crucial to take into consideration the users' profile features and characteristics, which again makes human labeling very difficult to scale.

% In order to obtain a dataset for training query intent, we leverage the search clicked-through log for getting labeled data. Based on the assumption that given results of different types on the top search result page, the clicked ones are more relevant and more likely to bear the intent of that result type than the ones that are not clicked, we associate the vertical type of the clicked results with the searched query. For example, given a user searched for "linkedin sales solutions" and clicked on a job posting with title "Senior Customer Success Manager, Talent Solutions" instead of \textit{people} or \textit{content} results, a \textit{job} intent label is assigned to this query. We also leverage the queries searched in verticals with lower traffic in order to alleviate the problem of imbalanced data even if these queries did not result in a click. For example, \textit{learning}, as a new search vertical, receives much lower traffic compared to verticals like \textit{job} and \textit{people}. E.g., query "ai cources" is searched within the vertical search in \textit{learning} instead of on the top page, is labeled with a learning intent.



% \subsection{Text Representation}
% \subsubsection{Convolutional Neural Networks (CNN)}
% Word embedding has seen a lot of success in solving text related tasks. It is essentially a process of transforming words into vector representations where words that have similar meanings tend to have a similar representation. The vector representations are of a predefined length, usually in tens or hundreds of dimensions. This makes the learned features a lot different than the bag of words representation, which is often sparse and highly-dimensional in practice.

% In practice, there are different approaches to learning the word representation or word embeddings.
% \begin{itemize}
% \item Learning the embeddings from scratch. It is possible to learn the word embeddings using our own domain specific text. This requires that we have a large set of data and could result in a longer training time.
% \item Reusing a pre-trained word embedding. Since quite a few word vector representations are available for free and provide great quality for representing words for a global vocabulary, it is often very efficient to reuse such pretrained word representations and adapt the model using our own text corpus.
% \end{itemize}

% We initialize the word vectors using GloVe word vector representations pre-trained on LinkedIn text data. It covers a vocabulary size of 400K and we chose to use vectors of size 100.
% The idea is to have the embedding layers be “trainable” during the model training phase. In this case, the GloVe word vectors are used as the initial “seeds” and then the embeddings are further fine-tuned using LinkedIn’s search data. As a result, the domain-specific similarities among text are captured and “embedded” in these vector representations.

% \begin{figure}
%   \includegraphics[width=80mm]{figure/qim-cnn.pdf}
%   \caption{Text feature extraction with CNN.}
%   \label{figure:qim-cnn-ft-ext}
% \end{figure}

% The query text representation is extracted with CNN, as illustrated in Figure \ref{figure:qim-cnn-ft-ext}. The convolution layers involve multiple filters of different heights. The width of the CNN filters is always same size as the whole embeddings, while the height of the filters is different—it represents how many words are covered by the filter. The main reason for using filters of different sizes is for the model to capture the n-gram information of the query. As illustrated in Figure 3, we use filters of height 2, 3, and 4 to capture bigram, trigram, and 4-gram information of the searched text. Max-pooling over time was done after each convolution layer. 

% \subsubsection{Contextualized Representation with BERT}
% CNNs are good at capturing the word ngrams patterns and modeling the spatial characteristics in text. BERT\cite{devlin2018bert} not only captures the static meaning of the words, but also integrates contextual features from both left and right, achieving state-of-the-art results in many classic NLP tasks. We describe our query text feature extraction with BERT in this section.

% Given a query, BERT takes a sequence of tokens as input and output the contextualized representation of the sequence. A special token \texttt{[CLS]} at the beginning of each sequence models the representation of the entire sequence and is used for classification tasks. In our word-level query intent classification model, given a query, we take the final hidden state of \texttt{[CLS]} as the representation of the query and extract the text features. 

% However, gaps still exist between academic research and industry applications, especially for the products that have stringent latency requirements. This major challenge motivates us to pre-train a BERT model with light-weight architectures and text corpus from LinkedIn (hence the name LiBERT). The probabilities of intents given a query need to be computed on-the-fly instead of precomputing as there are unique queries from different members searched each day. Given that GPU and TPU serving is not yet available at LinkedIn, the latency for computing the query intent outputs using the BERT-Base model from Google won’t satisfy the critical latency requirement. The LiBERT model has a simpler architecture than the smallest released models from the original BERT paper\cite{devlin2018bert}. 

% In addition to the benefit of low latency, pre-training the BERT model from scratch with LinkedIn data leverages the in-domain knowledge in the corpus, therefore should produce better relevance performance for downstream fine-tuning tasks. An example is that \texttt{LinkedIn}, \texttt{Pinterest} are both out-of-vocabulary words in Google’s BERT-Base model. These company names are generally important for LinkedIn search. 


% discuss more about libert?


% \begin{figure}
%   \includegraphics[width=70mm]{figure/qim-bert.pdf}
%   \caption{Text feature extraction with BERT.}
%   \label{figure:qim-cnn-ft-ext}
% \end{figure}

% \subsection{Query Tagging Features}
% Traditional hand-crafted features could be very useful for capturing explicit patterns in search queries. In the previous production, query tagging confidence scores are used as query features indicating how likely certain types of entities exist in a query. The entity tags of query tagging outputs consist of types that are highly correlated to the search verticals. The query tagging features and deep features are often complementary. For example, given a query with names that are outside of the word embedding vocabulary, query tagging could predict the confidence scores of it containing \textit{first name} and \textit{last name}. Therefore in the deep learning based models, we consider incorporating the traditional query tagging features.

% \subsection{Searcher Characteristic Features}
% In order to support personalized intent prediction and search blending, searcher characteristic features are also very important, especially for ambiguous queries where these features could be very beneficial. We use aggregated member search history features and member behavioral footprint features. 

% The member search history features capture the search characteristics and patterns in the past. These characteristics are good indicators for a member's search pattern and could give strong hints of the future ambiguous search queries. For example, \textit{history group search} aggregates the number of search initiated in group search vertical for a particular member. With the same searched query, e.g. "google cloud bay area", members with higher scores for this feature are more likely to be searching with a \textit{group} vertical intent than those with lower scores. In total, there are 21 history features capturing search history, search result views, search result actions in all 7 verticals.

% Member footprint behavioral footprint features include a various footprint characteristics in different products relating to the different search verticals. Job seeker intent response, as an example, models how likely a member is a job seeker. Including these features in modeling the query intent gives crucial hints on how likely the searcher is looking for \textit{job} results instead of \textit{people} results. 16 footprint features are used together with the member search history features.

% The member characteristic features (37 continuous features) are captured and aggregated daily and the model is trained based on the features gathered from the previous day. In production, if the searcher is not a member at LinkedIn and therefore does not have any past characteristic features as input to the model, a global average of the searcher features will be used.



% \subsection{Model Architecture}
% Both CNN- and BERT-based approaches share common components in query intent classification network architecture. After automatic extraction with CNN/BERT, the query representation vector is concatenated with the query tagging confidence score features and searcher characteristic features. A hidden layer is added on top of the concatenated vectors to capture the non-linear interactions among these features. A final classification layer with softmax output of size 7, which equals to the number of vertical intents, is used.
% The model architecture is illustrated in Figure . 

% CNN
% \textbf{Embedding layer.} We first have an embedding layer where each word inside a document is one-hot encoded. The dimension of the word vectors is 100. We also pad the document to a fixed length sequence, with longer sequences cropped and shorter sequences padded to the fixed length. Here the length of the sequences is also a tunable parameter. As discussed above, the initialization of the word vectors are done using GloVe pre-trained embeddings.

% \textbf{Convolution layers.} The convolution layers involve multiple filters of different heights. The width of the CNN filters is always same size as the whole embeddings, while the height of the filters is different—it represents how many words are covered by the filter. The main reason for using filters of different sizes is for the model to capture the n-gram information of the query. As illustrated in Figure 3, we use filters of height 2 and 3, to capture bigram and trigram information of the searched text. Max-pooling over time was done after each convolution layer.

% \textbf{Concatenated features.} After pooling, we concatenate the features generated from different filter heights.
% Fully connected layer. A fully connected layer with ReLU activation function is used after the concatenated layer. 

% \textbf{Softmax layer.} A fully connected softmax layer of size equals number of classes was used.

% \subsection{QIM-BERT}




% \section{Character-level Model for Typeahead Blending}
% For typeahead blending, we propose a character-level intent prediction model that provides the intent predictions on the fly as the users type in each character in a search query. The model architecture is described in this section.

% Modeling the intents of incomplete queries could be a challenging task. Word-level query classification has been widely used for text classification tasks in search. However, the nature of typeahead search is that most of the time users do not complete the entire search keywords, but type the prefixes then select the search results returned from the drop-down bar. In this case, a large number of words in the queries would be recognized as out-of-vocabulary words, which causes information loss. 

% \subsection{Character Embeddings}
% The input to our character-level model is a search query, equivalent to a sequence of characters. The query is first broken down to characters, including white spaces. Then the characters are encoded using the character-level vocabulary. 
% To capture the accurate information from the characters, we design the character level vocabulary as follows:
% \begin{itemize}
%     \item The vocabulary is extracted from the training dataset.
%     \item Each character is an entry in the vocabulary.
%     \item Spaces are replaced by a special token \texttt{[SPACE]}.
%     \item Special token \texttt{[UNK]} is used to represent the unknown (unseen) characters.
% \end{itemize}


% \begin{figure}
%   \includegraphics[width=85mm]{figure/iqi-lstm.pdf}
%   \caption{Model architecture for BiLSTM character-level intent prediction.}
%   \label{figure:iqi-lstm}
% \end{figure}

% We use an embedding layer at the input to project the sequence of characters into sequence embeddings through table lookup. The embeddings of the characters and special tokens are initialized randomly at the beginning of training and later updated during training.

% \subsection{Bidirectional LSTM}
% The motivation of using RNN is for its ability to capture and learn the sequence information of the characters. Compared with CNN used for classification tasks, the long distance dependencies of the characters in the queries could be better captured by RNNs. We use the Bidirectional LSTM network to model the prediction task. 

% The input query is first tokenized as a sequence of characters. The sequence of embeddings of the input is extracted through the embedding layer.
% The LSTM layer takes the embedding sequence as input. We use bidirectional LSTM meaning that there’s a forward and a backward LSTM layer. The output of the last step of both layers are concatenated together to form the output layer. The output layer is the representation of the input incomplete query.
% A fully connected layer is then used to add more non-linearity.
% Finally a softmax classification layer is used for the multi-class classification task over different intent labels.


% \subsection{Multilingual model}
% \label{section:multilingual}

% \begin{figure}
% \begin{subfigure}{0.23\textwidth}
% \includegraphics[width=\linewidth]{figure/iqi-multilingual-embed.pdf}
% \caption{Embedding.} \label{figure:iqi-embed}
% \end{subfigure}
% \begin{subfigure}{0.24\textwidth}
% \includegraphics[width=\linewidth]{figure/iqi-multilingual-concat.pdf}
% \caption{Concatenation.} \label{figure:iqi-concat}
% \end{subfigure}
% \hspace*{\fill} % separation between the subfigures
% \caption{The language feature embedding and concatenation scheme for character-level query intent model.} 
% \label{figure:iqi-multilingual}
% \end{figure}
% Search systems at LinkedIn experience a large amount of traffic in multiple countries with various spoken languages. In typeahead search, more than 30\% of the impression and action traffic is from languages other than English. Handling the performance gap between English and other languages is crucial for a good user search experience in typeahead. Instead of training per-language models, which are effort-consuming and difficult to scale. In this section, we describe our approach for designing a multilingual model for typeahead query intent prediction.

% Natural language understanding for different languages is an important topic. Traditionally, per-language models are trained separately and deployed into individual locales in production. However, it takes great effort to develop and maintain offline (data collection and model training) pipelines and online applications in production. In addition, lack of training data is a major problem for languages that do not receive lots of traffic. The proposed unified multilingual model tackles with these challenges when applying the query intent model across multiple languages. More specifically:

% The character-level approach is perfect for multilingual models, since the character vocabulary of all languages is much smaller than the word vocabulary.
% Languages with smaller number of training samples could benefit from other similar languages as data augmentation.


% In order to train a unified model that could be used for the product in different locales using different languages, we want to design the query intent model so that the language/locale information and features could be extracted and “embedded” in the query features.


% \subsubsection{Language Feature Embedding}

% The first approach is to concatenate the interface locale embedding to the query embedding and the concatenated embeddings feed through a BiLSTM to extract interface locale “embedded” query features, as shown in Figure \ref{figure:iqi-embed}. The embeddings of the interface locales are randomly initialized and together trained with the network.

% \subsubsection{Language Feature Concatenation}

% The second approach, illustrated in Figure \ref{figure:iqi-concat} is to use the BiLSTM layer for extracting query features from query embeddings, and then concatenate the interface locale embeddings to the last output state of the BiLSTM. In this case, the language features (interface locale embeddings) is concatenated with the query features extracted from the BiLSTM network.







\section{Experiments}
Experiments on both incomplete and complete query intent prediction models are discussed in this section. Performance comparison in both offline and online metrics are shown by relative differences instead of absolute values due to company policy. We also share our analysis in the scalability of these deep learning based models, as well as the online A/B testing performance of these models compared with production baselines. All the reported online metrics lift are statistically significant ($p<0.05$).


\subsection{Training Data Collection}
\label{section:label-data-collection}
Search click-through log is used for training data collection. For example, given that a user searched for \textit{linkedin sales solutions} and clicked on a job posting instead of a \textit{people} or \textit{content} page, a \textit{job} intent label is assigned to this query. Similarly, when a user typed an incomplete query \textit{face} and chose the \textit{facebook} company page, then a \textit{company} intent is inferred.

There are two advantages of using click-through data instead of human labeling: (1) Intent is subjective and ambiguous, therefore it is challenging for human annotators to infer the intent without enough background information of the searcher. (2) 
We are able to harvest millions of training samples with clickthrough log, which is not scalable from human annotation.

For both incomplete and complete intent models, we collected training data sampled from clicked-through log for a month. For train/dev/test dataset, we sampled  24M/50k/50k for complete query intent model. 
%Training the deep learning based models requires large amount of data. By carefully designing the logic to obtain labeled data, we're able to utilize millions of training samples, which benefits the learning of the complex models.
% First of all, a clear definition of search query intent is difficult to achieve. For queries like "stanford university", we could interpret this is the case where a user wants to find the school Stanford University. However, the user may also want to look for people who graduated from the university or who're working at Stanford. Therefore designing rules for labeling the queries with different intent classes is a challenging task. 
% Secondly, intent is subjective, meaning that the intent for queries could vary in users of different background or even the same users but under different circumstances.For example, a job seeker searching with query "linkedin machine learning" could have strong intent looking for job posting results, whereas a recruiter searching with the same query hopes to get more profile pages as results. This means when labeling search queries with vertical intents, it's crucial to take into consideration the users' profile features and characteristics, which again makes human labeling very difficult to scale.


%Based on the assumption that given results of different types on the search result page, the clicked ones more likely to match the intent of that result type than the ones that are not clicked, we associate the type of the clicked result with the searched query. 

% We also leverage the queries searched in verticals with lower traffic in order to alleviate the problem of imbalanced data even if these queries did not result in a click. For example, \textit{learning}, as a new search vertical, receives much lower traffic compared to verticals like \textit{job} and \textit{people}. E.g., query "ai cources" is searched within the vertical search in \textit{learning} instead of on the top page, is labeled with a learning intent.

%More specifically, typeahead incomplete queries are used for incomplete query intent prediction, while queries that are searched after user hit the "search" button are used for collecting the training data for complete query intent models.
 
\subsection{Incomplete Query Intent Prediction}

\begin{table}
\small
\caption{Offline performance comparison for different character-level models vs production baseline.}
\label{table:iqi-offline}
\begin{tabular}{lccc}
\toprule
\textbf{Model}     & \textbf{Accuracy}    & \textbf{F1 (people)}     & \textbf{F1 (company)}    \\
\midrule
% BoW\textit{--TODO}     & -          & -      & -   \\
Tri-letter & - & -  & -  \\
CNN-en               & $+4.14\%$ & $+2.69\%$ & $+11.39\%$ \\
LSTM-en            & $+7.11\%$  & $+4.46\%$ & $+20.36\%$  \\
\bottomrule
\end{tabular}
\end{table}

\subsubsection{Experiment Setting}
% \hfill\\
% We collected search query data fired from typeahead search specifically. The incomplete queries in this dataset is used to train the character-level model. It is very difficult to due to the fact that: 1) the dataset we’d use is very large containing months of training data, and 2) there could be ambiguity in interpreting the search queries for the vertical intents. Therefore we used clicked-through information to infer the users’ intents with the search queries. More specifically, when a user issues a typeahead search, for example \texttt{goog}, and clicks the company entity result \texttt{Google} from the drop-down list, we assign a \textit{company} intent to this query.

We collected search query data originated from typeahead search specifically. The train/dev/test dataset contains 46M/570k/570k samples.

We evaluate the performance for character-based CNN and LSTM models in the offline experiments. The baseline model is learnt using letter tri-gram bag-of-words features with a logistic regression classifier. 

In the CNN/LSTM based models, character embeddings of size 128, with a 500 vocabulary size are used. 
The characters in the vocabulary are extracted from the most frequent characters in the training data. The embeddings are randomly initialized at the beginning of training. We used 128 convolutional filters of size 3 for training the CNN model. 
In the Bidirectional LSTM model, the same character vocabulary is used as in the CNN model and the number of hidden units is 128.

\subsubsection{Offline Experiments}
%  \hfill\\
Both English and multilingual incomplete query models are investigated in offline experiments. 
 
\vspace{1mm}
\noindent\textbf{English model.}
The first set of experiments were conducted on English incomplete queries. Experimental results show that compared with the tri-letter model, the CNN-based model is able to achieve a better accuracy, which is mostly because of the fact that CNN could extract more abstract word pattern features than traditional bag-of-words features. As shown in Table~\ref{table:iqi-offline}, the Bidirectional LSTM network can further improve the performance (+7.11\% vs. +4.14\%), since LSTM can better model the long range character sequences. 

\begin{table}
\small
\caption{The size of the character vocabulary for incomplete query intent models.}
\label{table:iqi-vocab}
\begin{tabular}{lcccc}
\vspace{-1mm}
\toprule
\textbf{Model}   &\textbf{Vocab}    & \textbf{Accuracy}    & \textbf{F1 (\textit{people})}     & \textbf{F1 (\textit{company})}    \\
\midrule
Tri-letter          & - & - &-  & -\\
CNN-en                  & $70$ & $+4.09\%$  &  $+2.69\%$ & $+11.38\%$ \\
CNN-en                  & $500$ &  $+4.14\%$ & $+2.73\%$  & $+11.75\%$\\
LSTM-en                 & $70$ &  $+7.04\%$ & $+4.46\%$  & $+20.36\%$\\
LSTM-en                 & $500$ &  $+7.11\%$ & $+4.49\%$ & $+20.49\%$\\
\bottomrule
\end{tabular}
\end{table}

We also compare the impact of character vocabulary size for the deep learning models (Table \ref{table:iqi-vocab}). It is interesting to see that even using a small vocabulary (only 70 characters consisting of lower-case English characters and special characters), the accuracy is significantly higher compared with the baseline model.
%In general, using a larger vocabulary size results in slightly higher overall accuracy as well as individual f1 scores. But by comparing the performance in Table \ref{table:iqi-vocab}, even using s small vocabulary that contains only 70 characters consist of lower-case English characters and special characters, the accuracy is significantly higher compared with the baseline model.

\vspace{1mm}
\noindent\textbf{Multilingual model.} In the multilingual experiments, we first collect training data using a similar procedure on top 30 international locales, such as French, Portuguese, German, etc. The international locales are used as language feature in our multilingual model. The most frequent 10k characters are extracted as vocabulary.
% Besides the two approaches, we also experimented with a third approach, which is the combination of the previous two. This enables embedding the language features into the query features by appending the interface locale embeddings to the character embeddings, while also attaching to the query features extracted from the BiLSTM network.
% \subsubsection{LSTM-based Multilingual Model}

\begin{table}
\small
\caption{Multilingual models for character-level incomplete query intent.}
\label{table:iqi-multi}
\begin{tabular}{lcccc}
\toprule
\textbf{Model}       & \textbf{Accuracy}    & \textbf{F1 (\textit{people})}     & \textbf{F1 (\textit{company})}    \\
\midrule
LSTM-i18n                  & -  & -  & - \\
LSTM-i18n-embed            & $+0.67\%$ & $+0.44\%$  & $+1.34\%$  \\
LSTM-i18n-concat           & $+0.55\%$ & $+0.37\%$  & $+1.12\%$  \\
% LSTM-i18n-embed-concat     & $+0.67\%$ & $+0.45\%$  & $+1.36\%$  \\
\bottomrule
\end{tabular}
\end{table}

Table~\ref{table:iqi-multi} summarizes the performance of two different strategies discussed in Section~\ref{section:multilingual}. The language feature embedding method (LSTM-i18n-embed) outperforms the concatenation (LSTM-i18n-concat) method slightly. 
%The major difference of the two is that the first approach incorporates the language information into the characters whereas the second approach concatenate it on the query level. 
This might be that in LSTM-i18n-concat, the LSTM is aware of the language, hence generate a more meaningful embedding for the sequence. 
These experiment results suggest that both methods outperform the baseline model without language embedding injected. 
% We did not observe much gain from combining the two methods in LSTM-char-embed-concat.


We further compare the effectiveness of the multilingual models to the traditional per-language models. Table\ref{table:iqi-multi-single} shows the overall accuracy and per-language accuracy. The LSTM-per-lang is trained and evaluate on per-language datsets. LSTM is the multilingual model without language features added.  LSTM-i18n-embed is with language feature added to the character embeddings. The overall accuracy for the multilingual model is comparable to the per-language model. We also sampled 4 languages to show the individual performances. For French (fr), both multilingual models improved performance compared with the single language LSTM-i18n-per-lang model trained on French data only. This is true that for certain languages, multilingual helps the model to learn from other languages and generalize better to help predictions on the specific languages. From results in the other 3 languages, the multilingual models did not outperform the per-language models. This is often expected. But with the language feature embedded, we observed an increased accuracy compared to the LSTM  model. 
\begin{table}
\small
\caption{Multilingual model vs per-language models. } 
\label{table:iqi-multi-single}
\begin{tabular}{lccccc}
\toprule
Model & Overall &	fr &	de &	sv &   	da  \\
\midrule
LSTM-i18n-per-lang &	- &	- &	- &	-  & -\\
LSTM-i18n & $-0.65\%$ &  $0.28\%$   & $-0.84\%$   & $-1.87\%$ & $-1.24\%$	 \\
LSTM-i18n-embed & $0.02\%$ &	 $0.56\%$   & $-0.18\%$   & $-1.11\%$ & $-0.66\%$	 \\
\bottomrule
\end{tabular}
\end{table}

\subsubsection{Online Experiments}
% \hfill\\

% IQI online: both en_US and multilingual
\begin{table}
\small
\caption{Online performance comparison for character-level query intent prediction model in typeahead search vs production baseline (a linear model).}
\label{table:iqi-online}
\begin{tabular}{llc}
\toprule
\textbf{Model} & \multicolumn{1}{c}{\textbf{Metrics}} & \textbf{\% lift} \\
 \midrule
\multirow{3}{*}{LSTM-en (en)} & Search session success & +0.43\% \\
%  & Entity views (mobile) & +0.34\% \\
 & Average time to success (mobile) & -0.15\% \\
 \midrule
\multirow{2}{*}{LSTM-i18n-embed (non-en)} & Search session success & +0.86\% \\
 & Average time to success (mobile) & -0.19\%\\
\bottomrule
\end{tabular}
\end{table}

As shown in Table~\ref{table:iqi-online} English model (LSTM-en)/multilingual model (LSTM-i18n-embed) is tested in typeahead search production with English/non-English traffic, respectively. 
% The set of online metrics are slightly different compared with those from the word-level metrics as the performance of the incomplete queries are be measured from the session success perspective. 
The online business metrics measure the success criteria within the search sessions. 
Both models show significant performance gain for \textit{search session success}. An interesting observation is that the \textit{average time to success} on mobile is reduced for both models. A possible intuitive reason is that users are more likely to be interested in high quality results rendered in typeahead search when they are searching on mobile devices vs desktop. 
% The \textit{entity views}, which refers to the result view with a sufficiently long time, on mobile also shows $0.34\%$ lift for the LSTM-en model. 
\subsection{Complete Query Intent Prediction}
\label{section:complete-intent}
\subsubsection{Experiment Setting}
The word-level query intent models are learned from past query click-through logs. Following the procedures discussed in Section \ref{section:label-data-collection}, we collected queries from the past month: 24M records for training data and 50k for dev and test set. The intent classes include the major search result types in LinkedIn.  

% \subsubsection{CNN-baed Model}

% \subsubsection{BERT-baed Model}

\begin{table}
\small
\caption{Offline performance comparison for the word-level models vs production baseline.}
\label{table:qim-offline}
\begin{tabular}{lccc}
\toprule
\textbf{Model}     & \textbf{Accuracy}    & \textbf{F1 (\textit{people})}     & \textbf{F1 (\textit{job})}    \\
\midrule
LR     & $-2.4\%$          & $-3.9\%$      & $-8.34\%$   \\
LR-BOW & - & -  & - \\
\midrule
CNN-word                & $+6.40\%$ & $+1.36\%$ & $+17.35\%$ \\
CNN-char        & $+3.49\%$ & $-0.50\%$ & $+10.29\%$\\
LSTM-word              & $+6.69\%$  & $+1.47\%$ & $+17.99\%$  \\
LSTM-char           & $+4.63\%$ & $+0.23\%$ & $+13.46\%$  \\
\midrule
BERT-Base              & $+8.20\%$  & $+2.33\%$ & $+19.33\%$  \\
LiBERT              & $+8.35\%$  & $+2.46\%$ & $+20.60\%$  \\
\bottomrule
\end{tabular}
\end{table}
The input is word-level embeddings. The embeddings are initialized using GloVe\cite{pennington2014glove} word vector representations pre-trained on LinkedIn text data. It covers a vocabulary size of 100K with dimension 64. 

The production baseline model is a logistic regression model, with bag-of-words features, and user profile/behavioral features, etc. In the offline experiments, we first compare the performance among the deep learning models with the production baseline. Another baseline model to compare is a logistic regression model without the Bag-of-Words language features.

For the CNN-based model, we used 128 filters of height 3 (trigram) for the 1-D convolution. The hidden state size is 128 for the LSTM-based model. For both CNN and LSTMs, after the query embedding is generated, a layer of size 200 is used to capture the non-linear interactions between the query embedding and continuous traditional features.


\subsubsection{LiBERT Pre-training}
\label{section:libert-pretrain}

\begin{table}
\small
\caption{Model architecture comparison between LiBERT Google's BERT-Base.}
\label{table:libert-param}
\begin{tabular}{lcc}
\toprule
\textbf{BERT HParams} & \textbf{BERT-Base} & \textbf{LiBERT} \\
\midrule
Layers & 12 & 3 \\
Hidden size & 768 & 256 \\
Attention heads & 12 & 8 \\
\midrule
Total \#params &  110M & 10M  \\
\bottomrule
\end{tabular}
\end{table}


The LiBERT-baesed model is fine-tuned with a pre-trained BERT model with LinkedIn data.
% We used large amount of unlabeled text data tracked from different applications in LinkedIn. 
% The LiBERT model also has a light-weight network structure compared with Google's BERT-Base model. The detailed comparison of the two models are listed in Table\ref{table:libert-param}. 
The pre-training data include a wide variety of data sources across LinkedIn: search queries, user profiles, job posts, etc. The collected data for pre-training include around 1 billion words. 
% With the help of in-domain data, embeddings extracted are more meaningful towards LinkedIn applications than if we were to use the off-the-shelf BERT models.
A light-weight structure is used compared to the smallest model (BERT-Base) published in BERT \cite{devlin2018bert}. A comparison between BERT-Base and LiBERT is given in Table \ref{table:libert-param}. %In order to meet the online latency requirements, 3 transformer layers are used with hidden size equal to 256 and attention heads of 8. 
% Fine-tuned LiBERT based query intent models meet  inference latency requirement while BERT-Base model fails  by a large margin. Further details are discussed in Section \ref{section:scalability}.

\subsubsection{Offline Experiments}
% \hfill\\
Table \ref{table:qim-offline} summarizes the performance of different models.  
CNN/LSTM outperforms the baseline models, by $+6.40\%$/$+6.69\%$, respectively. 
% It is worth noting that the improvement of LSTM-word over CNN-word (+0.29\%) in complete queries (word sequences) is significantly smaller than that in incomplete queries (character sequence) (+2.97\% in Table \ref{table:iqi-offline}). It suggests that the long range dependency has smaller impact in complete word level queries than in incomplete character level queries. Therefore, we ramped the CNN model for online testing.
%This implies that the sequential information in the search queries is limited as LSTM has a similar performance compared with CNN, which extracts local spatial patterns. 



We further compared the performances of the complete query models in different token granularity and deep model types.
First, the word-level models outperforms character-level models consistently. This implies that for complete queries, word level representations captures more meaningful features than character sequences. Next, we compare the performance in LSTM and CNN models under different token granularity. More specifically, on word-level models, LSTM and CNN have similar performances. This implies that the useful sequential information is limited in the word sequences due to the short length of the queries and possibly the effectiveness of word-level information such as word meaning. This is further proved as when comparing the character-level models, LSTM outperforms CNN by a larger margin, meaning that longer range information is more useful in character sequence modeling. This is similar to the findings in incomplete query intent modeling experiments in , where we saw significant improvement from CNN to LSTM. The performance lift differences implies that the LSTM is more suitable in modeling the incomplete character sequences in typeahead than the complete queries in SERP.

We also experimented with character-level models for complete queries. As expected, word level models (CNN-word, LSTM-word) achieve much higher accuracy than character-level models (CNN-char, LSTM-char). 
% This further confirms our discussion to use word representations in modeling the full queries as accurate intent predictions is crucial to SERP blending.

BERT models (BERT-Base and LiBERT) can further improve the accuracy over CNN/LSTM  models. This should be attributed to that the contextual embeddings are able to disambiguate words under different contexts better. 



% \begin{table}
% % \small
% \caption{P1:The effect of filter window size for CNN-based word-level models.}
% \label{table:qim-cnn-window}
% \begin{tabular}{llccc}
% \toprule
% \textbf{Filter size}    & \textbf{Accuracy}    & \textbf{F1 (\textit{people})}     & \textbf{F1 (\textit{job})}    \\
% \midrule
% 3 &   &   & \\
% 2 &   &   & \\
% 4 &   &   & \\
% 2, 3, 4  &   &   & \\
% \bottomrule
% \end{tabular}
% \end{table}

\begin{table}
\small
\caption{The effect of different number of filters in CNN-based word-level models.}
\label{table:qim-cnn-filter}
\begin{tabular}{llccc}
\toprule
\textbf{\#Filters}     & \textbf{Accuracy}    & \textbf{F1 (\textit{people})}     & \textbf{F1 (\textit{job})}    \\
\midrule
32                   &  - & -  & -\\
64                  & $+0.16\%$  & $+0.09\%$  & $+0.30\%$ \\
128                   &  $+0.20\%$ & $+0.10\%$  & $+0.57\%$ \\
256                & $+0.29\%$  & $+0.15\%$  & $+0.61\%$\\
\bottomrule
\end{tabular}
\end{table}

\subsubsection{Online Experiments}
\label{section:scalability}
% \hfill\\

\begin{table}
\small
\caption{Online performance comparison for word-level complete query intent model vs production baseline in SERP blending.}
\label{table:qim-cnn-online}
\begin{tabular}{llc}
\toprule
\textbf{Model} & \textbf{Metrics} & \textbf{\% lift} \\
\midrule
\multirow{2}{*}{CNN-word} & CTR@5 for job results & +0.43\% \\
 & Job viewers & +0.36\% \\
\midrule
\multirow{3}{*}{LiBERT (vs. CNN-word)} & CTR@5 & +0.17\% \\
 & CTR@5 for job results & +0.51\% \\
 & SAT click & +1.36\% \\
\bottomrule
\end{tabular}
\end{table}

It is worth noting that even though the LSTM model performs slightly better than the CNN model, we proceed to implement the CNN model in online production. This is due to the fact that LSTM does not bring much relevance gain while introducing almost 2 times inference latency (Table \ref{table:latency}).

Table \ref{table:qim-cnn-online} shows the online metrics gain of CNN model over logistic regression. It improves two job search related metrics: the overall click-through rate of job postings at top 1 to 5 positions in the search result page (CTR@5 for Job Results), and total number of job search result viewers (Job  Viewers). This is because the F1 score of job intent is significantly improved (offline results in Table \ref{table:qim-offline}).

Later, we conducted online experiments of LiBERT over CNN (Table \ref{table:qim-cnn-online}). Since LiBERT can significantly improve the offline F1 score of people intent, and people search has a larger traffic than job search, overall search metrics (not limited to job results) are improved, including SAT clicks (the clicks on documents with a long dwell time), and CTR@5 over all documents.

%In addition, the LiBERT based models are deployed to online production for A/B testing. Overall, the deep learning based models improves the search quality as relevance related metrics show statistically significant gain. The \textit{CTR@5} metric measures the overall click-through rate at top 1 to 5 positions in the search result page. For the CNN-based model, \textit{CTR@5} for \textit{job} results improved by $0.43\%$, which suggests that the model provide a more accurate prediction of \textit{job} queries. Similarly, the overall \textit{CTR@5} and \textit{CTR@5 for job} results show improvement for the LiBERT-based model. 

%Besides the search clicks metrics, other careers related metrics and search session metrics also show significant lift. \textit{Job member viewers} gained $0.36\%$ with the CNN-word experiment. The \textit{SAT click} metric is short for \textit{SATisfied search click}, which measures the quality of the clicks from search. The satisfied search clicks are those from 1) actions from a connect, message, job apply, 2) result views with sufficiently long dwell time. The LiBERT model improved \textit{SAT click} metric by $+1.36\%$, indicating higher quality of search clicks as a result without violating online latency requirements. 



\subsection{Scalability}

%In the online serving stage of the query intent models, latency is the major challenge for productionization. 
% strict latency
%First of all, online pre-computation is not feasible as there are large number of unseen queries each day for large search engines. Therefore we have to load the models in memory and compute the intention predictions on-the-fly.  In Addition, query intent predictions are computed at the early stage of the search ecosystem: before document retrieval. Downstream tasks such as vertical selection and search ranking depend on the returned predictions. Therefore stringent latency requirements are enforced for the computation of the intent prediction algorithms. Both requirements call for finding a balance between model effectiveness and efficiency. 

%In the stage of incomplete query intent prediction, the production application tries to provide an early guess of the searcher's intent. The intent scores are calculated with each key stroke therefore the model needs to inference at a very fast speed. For the complete query intent prediction, although still at a strict latency requirement level, it's much more relaxed compared with the incomplete query intent scenario. 

In the online system, latency at 99 pencentile (P99) is the major challenge for productionization. For query intent, offline pre-computation of the frequent queries does not help, since the P99 queries are usually rare, and there are large number of unseen queries each day at LinkedIn search.

The latency comparison of the character-level models (CNN-char and LSTM-char) for incomplete queries is shown in Table \ref{table:latency}. Both CNN-char and LSTM-char models satisfy the latency requirements for typeahead search. We decide to ramp the LSTM based character model online as it yields a better accuracy.  % With the language feature added, the inference latency for the LSTM-char-embed multilingual model  does not increase much and is within production requirement.

In terms of complete queries, the CNN/LSTM models have even less latency, since number of words are generally smaller than number of characters. For BERT models, the latency increases significantly. It is worth noting that by pre-training a smaller BERT model on in-domain, we are able to reduce the latency from 53ms (BERT-Base) to 15ms (LiBERT), which meets the search blending latency requirement.

%In Section \ref{section:complete-intent}, we show that pre-training the in-domain BERT model (LiBERT) gives the benefit of improved relevance offline and online performance compared with CNN/LSTM or Google's BERT-Base models. It is worth noting that another major benefit by pre-training a more compact model greatly reduced the inference latency and therefore satisfying the latency requirements. Comparing the LiBERT models in Table \ref{table:latency}, by using a more compact model architecture, LiBERT increased the latency by 15ms, which is still within the production latency requirements. The BERT-Base query intent model, on the other hand, requires a much slower inference speed. 

% latency comparison


\begin{table}
\small
\caption{Latency comparison on different models at 99 percentile.}
\label{table:latency}
\begin{tabular}{llc}
\toprule
  & \textbf{Model} & \textbf{P99 Latency}  \\
\midrule
\multirow{3}{*}{Incomplete query intent} & Tri-letter  &  - \\
& CNN-char                   &  $+0.38ms$  \\
& LSTM-char                & $+2.49ms$  \\
& LSTM-char-embed               & $+2.72ms$ \\
\midrule
\multirow{4}{*}{Complete query intent} & LR-BOW  &  - \\
& CNN-word                  & $+0.45ms$   \\
& LSTM-word                & $+0.96ms$  \\
& BERT-Base                & $+53.2ms$  \\
& LiBERT                & $+15.0ms$  \\

\bottomrule
\end{tabular}
\end{table}
% \subsection{Online Experiments}
